Simple Delegated Choice

This paper studies delegation in a model of discrete choice. In the delegation problem, an uninformed principal must consult an informed agent to make a decision. Both the agent and principal have preferences over the decided-upon action which vary based on the state of the world, and which may not be aligned. The principal may commit to a mechanism, which maps reports of the agent to actions. When this mechanism is deterministic, it can take the form of a menu of actions, from which the agent simply chooses upon observing the state. In this case, the principal is said to have delegated the choice of action to the agent. We consider a setting where the decision being delegated is a choice of a utility-maximizing action from a set of several options. We assume the shared portion of the agent's and principal's utilities is drawn from a distribution known to the principal, and that utility misalignment takes the form of a known bias for or against each action. We provide tight approximation analyses for simple threshold policies under three increasingly general sets of assumptions. With independently-distributed utilities, we prove a $3$-approximation. When the agent has an outside option the principal cannot rule out, the constant approximation fails, but we prove a $\log \rho/\log\log \rho$-approximation, where $\rho$ is the ratio of the maximum value to the optimal utility. We also give a weaker but tight bound that holds for correlated values, and complement our upper bounds with hardness results. One special case of our model is utility-based assortment optimization, for which our results are new.

==> agreement.tex <==
In the example in Appendix~\ref{app:project_selection}, a firm (the principal) must select one of several projects for a team (the agent) to undertake. While both the team and firm benefit from undertaking a project, only the team observes and internalizes the project-specific costs. Hence, the benefits of the projects are a natural choice for the value matrix $V$, and the state-specific effort costs paid by the agent serve as the distortion $D$, yielding decomposition coefficients $a_1=a_3=1$, $a_2=0$, and $a_4=-1$. Note that because the value of each project is known in advance, all columns of $V$ are identical.  This will often be the case when the source of distortion are effort costs that depend on information which is unknown to the principal, but where benefits are known to all parties in advance. We refer to this condition as \emph{restricted value}. Formally:

\begin{definition}
An instance of delegation with utility decomposition $(a_1,a_2,a_3,a_4,V,D)$ satisfies \emph{restricted value} if all columns of $V$ are identical.
\end{definition}

Since each column of $V$ is identical, for the rest of this section we let $v_i$ denote the value which populates the $i^{\text{th}}$ row of $V$, i.e. the value associated with action $i$.

An natural question to ask is whether the delegation under restricted value exhibits as rich a structure as restricted distortion did above. In this section, we show that this is not the case. We do so in two ways. First, we show the perhaps surprising result that in the presence of an outside option, delegation is still as hard as the general case. We prove this result in Appendix~\ref{app:valuehard}. Second, we show that with no outside option, the delegation problem becomes trivial: the principal should just pick their favorite action and impose it on the agent.

%% old text
%In managerial decisionmaking, this can appear when effort costs for different projects or implementation choices are known only to the agent (and experienced only by the agent), while both the agent and principal agree on the value of the various options to the firm. More generally, the restricted value condition holds when the costs of actions to either the agent or the principal are more sensitive to the state than the mutual benefit the players experience. We formalize the condition below:
%\begin{assumption}[Restricted Value]\label{ass:value}
%The \v\ matrix $V$ is independent of the states and only a function of the actions. In other words,
%$$v_{ij}=v_i\quad \forall j\in S.$$
%\end{assumption}
%Note that Assumption~\ref{ass:value} imposes no sign restrictions on either the \v\ matrix $V$ or the \d\ matrix $D.$ The main result of this section holds regardless of the signs of these matrices.

 To characterize delegation in the absence of an outside option, we derive an intuitive consequence of the restricted value condition. Because the state only affects the utilities of the agent and principal in a way that causes their preferences to diverge, it follows that any time the agent would change their decision based on the state, the principal would prefer the opposite. Moreover, if the agent was restricted in their strategy to choose each action with a certain frequency, they would allocate their action ``quotas'' in a way that exactly minimizes the principal's utility over all strategies satisfying the frequency restriction. We formalize this notion as follows:

\begin{definition}
Given a delegation set $A$, the \emph{frequency} of an action $a$ under $A$, denoted $q_a$, is the probability the agent takes action $a$, given by $\sum_{s\in S}p_s\mathbbm{1}[g(A,s)=a]$.
\end{definition}

\begin{definition}\label{def:reassign}
Given a delegation set $A$ and action frequencies $(q_1,\ldots,q_m)$ for $A$, an \emph{action reassignment} is an $m\times n$ matrix $R$ such that:
\begin{enumerate}
	\item For all $a\in \Omega$ and $s\in S$, $r_{as}\geq 0$.	
	\item For all $s\in S$, $\sum_{a\in \Omega}r_{as}=1$.
	\item\label{pt:quota} For all $a\in \Omega$, $\sum_{s\in S}p_sr_{as}=q_a$.
\end{enumerate} 
\end{definition}

Action reassignments represent feasible solutions to the following thought experiment: given a delegation set $A$, allow the principal to observe the state and assign actions in $A$ to states in a probabilistic fashion, subject to the constraint that the frequency of each action is the same as if the agent was choosing the action for each state. Because the only state-dependent part of the agent's utility is exactly misaligned with that of the principal, any reassignment of actions to states is preferable for the principal to the assignment selected by the agent. This can be interpreted as an ``anti-alignment'' condition, and functions as an obverse to the alignment condition discussed in e.g. \citet{frankel2014aligned}. Formally:

\begin{lemma}\label{lem:perms}
If utilities satisfy the restricted \v\ condition, then for any delegation set $A$ and any action reassignment $R$, the principal's utility satisfies:
\begin{equation}
\sum_{s\in S}p_s\Up(g(A,s),s)\leq \sum_{s\in S}\sum_{a\in \Omega}p_sr_{sa}\Up(a,s)
\notag
\end{equation}
\end{lemma}
\begin{proof}
In state $s$, faced with action set $A$, the agent chooses action $g(A,s)$. An alternate, randomized strategy the agent could employ would be to choose action $a$ in state $s$ with probability $r_{as}$, for every state $s$. This deviation is suboptimal for the agent, so we have:
\begin{equation}\label{eq:agentuitls}
	\sum_{s\in S}p_s v_{g(A,s)}+	\sum_{s\in S}p_sD({g(A,s),s})\geq 	\sum_{s\in S}p_s\sum_{a\in \Omega} r_{as}v_{a}+\sum_{s\in S}p_s\sum_{a\in \Omega}r_{as}D({a,s}).
\end{equation}
Note that the first term on each side of (\ref{eq:agentuitls}) is only a function of the number of times each action is taken under the agent's optimal strategy. But note that by condition (\ref{pt:quota}) of Definition~\ref{def:reassign}, action reassignments preserve these frequencies. Hence,
\begin{equation}\label{eq:agentval}
\sum_{s\in S} p_sv_{g(A,s)}=\sum_{a\in \Omega}q_av_a=\sum_{s\in S}p_s\sum_{a\in \Omega}r_{as}v_a
\end{equation}
It follows that the agent prefers taking $g(A,s)$ in state $s$ to $g(A,\pi(s))$ solely because of the component of their utility which is misaligned with the principal's, i.e.:
\begin{equation}\label{eq:agentprice}
\sum_{s\in S}p_sD({g(A,s),s}) \geq \sum_{s\in S}p_s\sum_{a\in \Omega}r_{as}D({a,s}).
\end{equation}
Combining (\ref{eq:agentval}) and (\ref{eq:agentprice}) yields the following inequality, which is equivalent to the lemma:
\begin{equation}
\sum_{s\in S}p_s v_{g(A,s)}-	\sum_{s\in S}p_sD({g(A,s),s})\geq 	\sum_{s\in S}p_s\sum_{a\in \Omega} r_{as}v_{a}-\sum_{s\in S}p_s\sum_{a\in \Omega}r_{as}D({a,s}).
\end{equation}
\end{proof}

\begin{theorem}\label{thm:valrestrict}
If utilities satisfy the restricted \v\ condition, then there is an optimal delegation set which is a singleton.
\end{theorem}
\begin{proof}
Let $A^*$ be an optimal delegation set, and let $(q_1^*,\ldots q_m^*)$ denote the action frequencies under $A^*$. It is a feasible action reassignment to take action $i$ with probability $q_a^*$, regardless of the state. That is, define an action reassignment $R^*$ such that $r^*_{as}=q_a^*$ for all $s\in S$. By Lemma~\ref{lem:perms}, we have:
\begin{align*}
\sum_{s\in S}p_s\Up(g(A^*,s),s) &\leq \sum_{s\in S}p_s\sum_{a\in \Omega}r_{as}^*\Up(a,s)\\
&= \sum_{s\in S}p_s\sum_{a\in \Omega}q_a^*\Up(a,s)\\
&= \sum_{a\in\Omega}q_a^*\sum_{s\in S}p_s\Up(a,s)
\end{align*}

%% Old analysis fragment
%Since $\pi$ is selected uniformly at random, the principal's expected utility from selecting actions according to $\pi(s)$ is only a function of the frequency with which each action is selected according to $g(A^*,s)$. In other words, let $\#a$ denote the number of states in which it is optimal for the agent to select $a$ from $A^*$. We have:
%\begin{align*}
%\mathbb E_{\pi}\left[\sum_{s\in S}\Up(g(A^*,\pi(s)),s)\right]&= \frac{1}{n}\sum_{s\in S}\sum_{a\in\Omega}\# a\cdot \Up(a,s).\\
%&=\sum_{a\in \Omega}\frac{\#a}{n}\sum_{s\in S}\Up(a,s).
%\end{align*}

The last line above can be interpreted as the expected utility from choosing an action $a$ with probability $q_a^*$ and playing this action in every state. Since this is at least the principal's utility from allowing the agent to choose from the set $A^*$, it follows that there must be an action $a^*$ such that playing $a^*$ in every state yields at least as much utility as allowing the agent to choose from $A^*$. This proves the theorem.
\end{proof}

Note that scenarios in which Theorem~\ref{thm:valrestrict} holds explanatory power often do not appear as mechanism design. That is, a principal for whom the optimal solution is a single action regardless of state need not delegate authority to an informed agent in the first place. In fact, Theorem~\ref{thm:valrestrict} suggests that it may be optimal to do away with the informed agent all together. It states that what appears as a single-agent problem may only appear so because of incentive problems the principal seeks to avoid.

==> auction.tex <==
We now analyze the first of two cases in which we assume the disagreement between the agent and principal is independent of the state. In other words, the mutual value to both agents of each action is more sensitive to the state than the costs which cause incentives to diverge. We additionally assume that the distortion matrix is nonnegative. Consequently, disagreement between the agent and principal takes the form of an action-specific, state-independent distaste for certain actions on the part of the agent, and a taste for certain actions on the part of the principal. Some settings where this assumption is satisfied include the assortment selection problem of Example~\ref{ex:labor} and managerial decisionmaking where the subordinate's labor or effort cost for each project or implementation decision is relatively insensitive to the state. We may formalize our assumption as:

\begin{assumption}[Restricted Distortion, Negative Bias]
The \d\ matrix $D$ is independent of the states and only a function of the actions. In other words,
$$d_{ij}=d_i\geq 0 \quad \forall j\in S.$$
\end{assumption}

Our conclusions under this assumptions are threefold. First, we prove that the delegation problem under this assumption is APX-hard. This suggests that the optimal mechanism can be extremely complex. We then present two analyses of threshold policies for the principal. In other words, the principal chooses a value $\underline d$ and allows the agent to select only actions $i$ such that $d_i\geq \underline d$. 
%TODO: Offer a real-life interpretation of threshold policies.
Our first result shows the best of the highest-distortion action and the full set of actions (i.e. the two trivial thresholds) is a 2-approximation. We then offer an improved analysis, in which we show that with low numbers of states, there exists a threshold policy which improves the principal's approximation guarantee. We show that both of these analyses are tight. We begin with our hardness result.



%Unlike the restricted \v\ case, the problem now differs depending on which player (principal or agent) considers $D$ as penalty and which one observes it as reward. In this section we consider the first variant of the problem, which we will refer to as \emph{\auction}, while the other variant is studied Section~\ref{sec:healthcare}. In \auction\ problem, we assume
%\begin{equation}
%\Up=V+D,\quad \Ua=V-D,
%\end{equation}
%where $V$ and $D$ are both nonnegative matrices. \\
%\red{TODO: motivating example / maybe explain the auction scenario in more details}
%%In this section, we may refer to $P$ as price (payment) for the agent and revenue for the principal.
\begin{theorem}
\label{thm:APX_auction}
With restricted \d\ and negative bias, the principal's delegation problem is APX-hard.
\end{theorem}

\begin{proof}
We give a reduction from the bounded degree vertex cover problem, i.e., the vertex cover problem on graphs with degree at most $B$ (constant). This problem is known to be APX-hard \cite{clementi1999improved}. Consider an instance of the bounded degree vertex cover problem $\Gt=(\Vt,\Et)$ with $\nt$ nodes and $\mt$ edges (where $\mt\leq B\cdot\nt/2=\O(\nt)$).\footnote{Again to distinguish between the parameters of the vertex cover instance and the delegation instance, we use tilde ($\sim$) for the graph instance.} We construct an instance of the \auction\ problem with $\mt+\nt$ states and $\nt+1$ actions. For each node $i$, there is an action $a_i$, with an additional ``default'' action $a_0$. Regarding states, there is a state $s_e$ for each edge $e=\{i,j\}$, whose value is $5$ only for actions $a_i$ and $a_j$ (two ends of that edge), $2$ for the default action, and $0$ for all other actions. There is also a state $s_i$ for each node $i$, whose value is $2$ only for $a_i$ and $a_0$ (default action), and $0$ for all other actions. Moreover, the only action with non-zero \d\ is the default action with $d_0=1$.

We claim that the optimal solution of the \auction\ problem produces a utility of $5\mt+3\nt-\kt$ for the principal, where $\kt$ is the size of the smallest vertex cover of $\Gt$. To see this, first note that any solution $\St \subseteq \Vt$ can be improved by including $a_0$, since $a_0$ has the biggest \d. Any time the agent would choose $a_0$, it is the optimal choice for the principal as well. We therefore only consider solutions containing $a_0$.

Now if $\St$ is a vertex cover of $\Gt$ with $\abs{\St}=\kt$, consider the corresponding \auction\ solution where the principal allows actions $\{a_i: i\in \St\}\cup\{a_0\}$. In all the states corresponding to edges, the agent will pick the action corresponding to one end of that edge (one is guaranteed to be in the cover $\St$) to get a utility of $5$ compared to $2-1$ achievable from the default action. This choice will also generate utility of $5$ for the principal, which makes $5\mt$ in total. For the states $s_i, i\in \St$ the agent will pick action $a_i$ which generates the utility of $2$ for both principal and agent. This will make $2\kt$ in total. Finally, for states $s_i,i\in \Vt\backslash\St$ the agent picks the default action which generates a utility of $2-1$ for himself but $2+1$ for the principal. This will give $3(\nt-\kt)$ in total. Summing up the utilities will give $5\mt+3\nt-\kt$.

For the converse, consider an optimal solution $A$ to the \auction\ problem. We show that the nodes corresponding to the actions in $A$ (excluding the default action) induce a vertex cover; otherwise the solution can be improved. Assume that there exists an edge $e=\{i,j\}$ where neither $a_i$ nor $a_j$ is allowed in $A$. If we add action $a_i$ to $A$, the principal gets a utility of $5$ in state $s_e$, compared to current utility of $3$ from the default action. On the other hand, the utility of the principal decreases in state $s_i$ from $3$ to $2$. So the total utility of $A\cup\{a_i\}$ is at least one more than $A$ which contradicts the optimality of $A$. Therefore $A$ should be a vertex cover (plus default action). This in turn implies that the utility is at most $5\mt+3\nt-\kt$ where $\kt$ is the size of the minimum vertex cover.

Since $\mt=\Theta(\nt)$ and the minimum vertex cover has size at least $\mt/B=\Omega(\nt)$, a constant factor gap in the bounded degree vertex cover problem translates into a constant factor gap in the optimal solution of the \auction\ problem, which yields the desired APX-hardness result. 
\end{proof}

We now study the approximate optimality of threshold policies under the restricted \d\, negative bias assumption. Recall the definition of utilities in the \auction\ problem. We see that
\begin{equation}
\label{eq:auction_intuition}
\Up=V+D=\underbrace{(V-D)}_\text{Agent's utility}+2D
\end{equation}
We consider the best of two policies: a policy which maximizes the agent's utility, and a policy which maximizes the principal's utility from distortion. To maximize the agent's utility, one can simply allow all the actions ($\Omega$) and the agent will maximize their utility. On the other hand, to maximize the \d, the principal should choose the single action with highest \d. In that case, the agent should pick that high-\d\ action in every single state, which maximizes the total \d. The principal's utility is a weighted combination of the two, which we know how to optimize individually. The approximation algorithm for the \auction\ problem is therefore to simply try both mentioned subsets of actions and pick the one that maximizes the principal's utility. We describe this policy formally in Algorithm~\ref{alg:auction}. We formalize our conclusion below:\footnote{We use the notion of $\alpha$-approximation algorithm as an algorithm whose output $APX$ satisfies $\alpha\cdot f(APX)\geq f(OPT)$, where $OPT$ is the optimal solution. Hence, all our approximation ratios are greater than one.}
%============= Algorithm ============
\begin{algorithm}[t]
	\SetAlgoNoLine
	\KwIn{Set of actions $\Omega$, set of states $S$, \v\ ($V$) and \d\ ($D$) matrices.}
	\KwOut{Set of actions $A$ that approximately maximizes $f(A)$.}
	$\Up=V+D$, $\Ua=V-D$.\\
	Set $A_1\gets \Omega$.\\
	Set $A_2\gets \{i\}$ where $i=\argmax_{i\in \Omega} d_i$.\\
	{\bf Return} $\argmax_{A\in \{A_1,A_2\}} f(A)$.\\
	\caption{Simple Threshold Policy for Negative Bias}
	\label{alg:auction}
\end{algorithm}
%=================================
\begin{theorem}\label{thm:simpleauction}
Algorithm~\ref{alg:auction} is a $2$-approximation algorithm under the \auction\ assumption with restricted \d\ matrix $D$.
\end{theorem}

\begin{proof}
Let $A_1$ and $A_2$ be defined as in Algorithm~\ref{alg:auction}, and $OPT$ be an optimal \auction\ solution. We have $\Up=\Ua+2D$ from \eqref{eq:auction_intuition}. For $A_1$, we can obtain a lower bound on the principal's utility by dropping the term that comes from the \d:
\begin{equation}
\notag
f(A_1)=\sum_{s\in S} \Up(g(A_1,s),s)\geq \sum_{s\in S} \Ua(g(A_1,s),s)\geq \sum_{s\in S} \Ua(g(OPT,s),s),
\end{equation}
where we used the non-negativity of the \d\ matrix in the first inequality. The second inequality comes from the fact that $A_1$ allows all the actions, hence the agent achieves a higher utility in every single state. On the other hand, we have the following lower bound for $A_2$:
\begin{equation}
\notag
f(A_2)=\sum_{s\in S} \Up(g(A_2,s),s)\geq 2\sum_{s\in S} D(g(A_2,s),s)\geq 2\sum_{s\in S} D(g(OPT,s),s),
\end{equation}
where the first inequality comes from the non-negativity of utilities, and the second one is due to the fact that $A_2$ is a singleton that has highest \d.

Adding the two lower bounds, completes the proof:
\begin{equation}
\notag
\max\{f(A_1),f(A_2)\}\geq \frac{1}{2}\big(f(A_1)+f(A_2)\big)\geq \frac{1}{2}f(OPT).
\end{equation}
\end{proof}

\subsection{Improved approximation algorithm}
Algorithm~\ref{alg:auction} is very simple; from the set of all $m$ threshold policies (or $2^m-1$ menus overall), it considers only two candidates. We now offer a more refined analysis of the set of threshold policies, and show that there exists a policy (not necessarily the two considered by Algorithm~\ref{alg:auction}) with approximation ratio $2-\frac{1}{n}$. This implies a better approximation algorithm for the principal: try every threshold policy, and adopt the best. We formalize this algorithm in Algorithm~\ref{alg:auction2}.
%
%\ We now we show how to improve the approximation ratio to $2-\frac{1}{n}$ by considering more subsets of actions. This new algorithm is still simple, as it considers at most $m$ different subsets. The idea of the algorithm is as follows. Again we start by considering the entire set of actions $\Omega$. Without loss of generality, assume that the actions are sorted based on the \d. In case that $f(\Omega)$ is not big enough, instead of removing all $m-1$ first actions (which leaves us with the singleton of highest \d), we remove actions one by one (starting from smallest \d). Clearly after $m-1$ steps we will get $A_2$ (see Alg.~\ref{alg:auction}), but it is possible that one of the intermediate subsets generates a better utility for the principal. Without the sorting assumption, the algorithm can be written as Algorithm~\ref{alg:auction2}.
%============= Algorithm ============
\begin{algorithm}[t]
	\SetAlgoNoLine
	\KwIn{Set of actions $\Omega$, set of states $S$, \v\ ($V$) and \d\ ($D$) matrices.}
	\KwOut{Set of actions $A$ that approximately maximizes $f(A)$.}
	$\Up=V+D$, $\Ua=V-D$.\\
	\For{each $k\in \{1,2,...,m\}$}{
	$threshold=d_k$.\\
	Set $A_k\gets \{i\in \Omega:d_i\geq threshold\}$.
		}
	Let $\mathcal{A}\coloneq\{A_1,...,A_m\}$.\\
	{\bf Return} $\argmax_{A\in \mathcal{A}} f(A)$.\\
	\caption{Improved Threshold Policy for Negative Bias}
	\label{alg:auction2}
\end{algorithm}
%=================================
\begin{theorem}
\label{thm:auction2}
Algorithm~\ref{alg:auction2} is a $(2-\frac{1}{n})$-approximation algorithm under the \auction\ assumption with restricted \d\ matrix $D$.
\end{theorem}

\begin{proof}
Let $OPT$ be an optimal solution, and define $a_i$ to be the index of action chosen by the agent, in the state $i$, given that he is allowed the actions in $OPT$. Let $d_0$ be the minimum \d\ in $OPT$. Without loss of generality, we can assume that the corresponding action is taken in at least one state, otherwise we can remove it without changing the optimal utility. Therefore we can write,
$$d_0=\min_{i\in OPT}d_i=\min_{i\in S}d_{a_i}.$$

Let $APX$ be the subset of actions within \d\ range of $[d_0,d_\text{max}]$, where $d_\text{max}$ is the highest \d\ in $\Omega$. Although we do not know $d_0$, the algorithm is guaranteed to find $APX$ at some iteration. Let $b_i$ be the index of action taken in state $i$, given that the agent is allowed to pick actions in $APX$. 

We show that if the agent picks a higher \d\ compared to the optimal solution (i.e., $d_{b_i}\geq d_{a_i}$) while the action $a_i$ is allowed, the principal is guaranteed to get a utility as big as the optimal solution in that particular state $i$. On the other hand, if the agent picks a lower \d, we show that the principal loses at most twice the \d\ difference (i.e., $2(d_{a_i}-d_{b_i})$). To show this, note that we have:
\begin{equation}
\label{eq:auc_agent}
v_{b_i,i}-d_{b_i}\geq v_{a_i,i}-d_{a_i},
\end{equation}
because $a_i\in APX$ (by choice of $d_0$), but the agent decided to pick $b_i$. This inequality can be re-written as 
$$v_{b_i,i}+d_{b_i}\geq v_{a_i,i}+d_{a_i}-2(d_{a_i}-d_{b_i}),$$
which justifies both cases mentioned above. Summing up this inequality over all states, we can form the utility of the principal in both optimal and approximate solutions:
$$\sum_{i\in S} (v_{b_i,i}+d_{b_i})\geq \sum_{i\in S} (v_{a_i,i}+d_{a_i})-2\sum_{i\in S} (d_{a_i}-d_{b_i}).$$
Therefore,
\begin{equation}
\label{eq:auc_loss}
APX\geq OPT-2\sum_{i\in S} (d_{a_i}-d_{b_i}),
\end{equation}
where we abused notation to write $OPT$ instead of $f(OPT)$ (same for $APX$).

Next, we have to bound the \d\ differences. By non-negativity of \d, any term $d_{a_i}-d_{b_i}$ is at most $d_\text{max}$. Moreover, $d_{a_i}-d_{b_i}$ is non-positive for at least one of the states. This is because $d_{b_i}\geq d_0$ (for all $i\in S$), and $d_0=d_{a_{i'}}$ for one particular state $i'$. In conclusion,
$$\sum_{i\in S} (d_{a_i}-d_{b_i})\leq (n-1)d_\text{max}.$$
Using this bound in \eqref{eq:auc_loss}, we get
\begin{equation}
\label{eq:auction_APX}
APX\geq OPT-2(n-1)d_\text{max}.
\end{equation}
In parallel, consider the singleton solution of highest \d. In that case, the agent is forced to pick that high-\d\ action in every single state. By non-negativity of utilities, the value of that action is at least $d_\text{max}$ in every state, generating the minimum utility of $2d_\text{max}$ for the principal. If we denote this singleton solution by $APX'$, we have
\begin{equation}
\label{eq:auction_APX'}
APX'\geq 2nd_\text{max}.
\end{equation} 
The final step is to take a weighted average of \eqref{eq:auction_APX} and \eqref{eq:auction_APX'}, as the better of the two will be better than the average. We multiply the inequalities by $\frac{n}{2n-1}$ and $\frac{n-1}{2n-1}$, respectively, and add them together.
$$\max{\{APX,APX'\}}\geq \bigg(\frac{n}{2n-1}\bigg)APX+\bigg(\frac{n-1}{2n-1}\bigg)APX'\geq \bigg(\frac{n}{2n-1}\bigg)OPT=\frac{OPT}{2-1/n}.$$
\end{proof}

In Appendix~\ref{supp:lower_bound}, we prove that the analysis of Theorem~\ref{thm:auction2} is tight: there exist instances where the best threshold policy achieves an approximation ratio of $2-1/n$. Since Algorithm~\ref{alg:auction2} always weakly outperforms Algorithm~\ref{alg:auction}, this implies that the analysis of Algorithm\ref{alg:auction} is tight as well.

%\paragraph{Discussion: Assortment Optimization} In the unit-demand assortment optimization problem, a seller considers which items to offer from a set of pre-priced items to a buyer with unknown value, who seeks to buy a single item. The results of this section have implications for welfare maximization in the unit-demand assortment allocation model, where the seller seeks to maximize the expected value of the buyer for the item purchased. Theorem~\ref{thm:APX_auction} implies that when the buyer's values for items are correlated, the welfare maximization problem is APX-hard. Moreover, Theorems~\ref{thm:simpleauction} and~\ref{thm:auction2} give 2-approximation algorithms in the case where the prices are sufficiently low (recall that we require $U_A$ to have only nonnegative entries).

==> decomposition.tex <==
We now turn to the main set of sassumptions structuring our results. In our discrete delegation model, one may easily decompose the principal's and agent's utility matrices to isolate the portion of their utility which is mutual, and the portion which is derived from player-specific distortion of utilities. Formally:

\begin{definition}
Given an instance $(U_P,U_A)$ of the delegation problem, a \emph{utility decomposition} for $(U_P,U_A)$ is given by constants $a_1$, $a_2$, $a_3$, and $a_4$ and matrices $V$ and $D$ such that $U_P=a_1V-a_2D$ and $U_A=a_3V+a_4D$. We refer to $a_1$, $a_2$, $a_3$, and $a_4$ as the \emph{decomposition coefficients} of $(a_1,a_2,a_3,a_4,V,D)$, $V$ as the \emph{value matrix}, and $D$ as the \emph{distortion matrix}.
\end{definition}

For any decomposition coefficients (as long as $a_1a_4+a_2a_3\neq 0$) we may obtain a corresponding utility decomposition by setting
\begin{equation*}
\begin{aligned}
V&=(a_1a_4+a_2a_3)^{-1}(a_4U_P+a_2U_A)\\%\notag
D&=(a_1a_4+a_2a_3)^{-1}(-a_3U_P+a_1U_A).
%\label{eq:algebra}
\end{aligned}
\end{equation*}

Note that the outside option utilities may also be decomposed into value and distortion, e.g. by writing $d_0=(U_P(0)-U_A(0))/2$ and $v_0=(U_P(0)+U_A(0))/2$ for coefficients $a_1=a_2=a_3=a_4=1$.


\subsection{Restricted Distortion}
As noted in the introduction, many settings admit utility decompositions where distortion captures monetary transfers or other action-specific sources of biases. Below, we summarize two assumptions on an instance's utility decomposition which capture these settings.

\begin{definition}
	An instance of delegation with utility decomposition $(a_1,a_2,a_3,a_4,V,D)$ satisfies \emph{restricted distortion} if all columns of $D$ are identical. 
\end{definition}

The procurement setting of Example~\ref{ex:procurement} satisifes restricted distortion, with the firm's benefits as $V$ and monetary costs $D$, yielding decomposition coefficients of $a_1=a_2=a_3=1$ and $a_4=0$. All random utility models in assortment optimization also satisfy restricted distortion, items' prices serving as distortion. For notational convenience, for a given action $a$ we will denote by $d_a$ the value populating the $a$th row of the distortion matrix $D$, and we will refer to $d_a$ as the \emph{distortion of action $a$}. Under restricted distortion, the principal may employ a simple threshold heuristic as their delegation set. Formally, we say the principal uses a {\em threshold policy} with threshold $t$ if the delegation set satisfies $A=\{a\in\Omega\,|\,d_a\leq t\}$. In the subsequent sections, we study the approximate optimality of threshold policies.

\subsection{Independent Values}

In addition to restricting each action's distortion, we make the further assumption that each action's value is drawn independently of other values. This is in line, for example, with a large portion of the literature on assortment optimization, where a common assumption is that the agent chooses an item according to a multinomial logit model. Since independently distributed values renders the number of states exponentially large, we abandon the value matrix notation under independence. We instead take $F_1,\ldots, F_n$ to be the respective marginal distributions for the values $v_1,\ldots, v_m$ of actions $\{1,\ldots, m\}$.


%in which the value or distortion matrix exhibit considerable structure. In the example in Appendix~\ref{app:project_selection}, a firm (the principal) must select one of several projects for a team (the agent) to undertake. While both the team and firm benefit from undertaking a project, only the team observes and internalizes the project-specific costs. Hence, the benefits of the projects are a natural choice for the value matrix $V$, and the state-specific effort costs paid by the agent serve as the distortion $D$, yielding decomposition coefficients $a_1=a_3=1$, $a_2=0$, and $a_4=-1$. Note that because the value of each project is known in advance, all columns of $V$ are identical.  This will often be the case when the source of distortion are effort costs that depend on information which is unknown to the principal, but where benefits are known to all parties in advance. We refer to this condition as \emph{restricted value}. Formally:

%\begin{definition}
%An instance of delegation with utility decomposition $(a_1,a_2,a_3,a_4,V,D)$ satisfies \emph{restricted value} if all columns of $V$ are identical.
%\end{definition}



%
%
%The restricted distortion and restricted value conditions still capture a variety of settings of interest (and in particular those for which existing models are ill-suited). In what follows, we study the effectiveness of simple delegation policies under each condition. In Section~\ref{sec:res_agreement}, we show that under the restricted value condition, an extremely simple policy is always optimal: pick the best single action and force the agent to take it. Therefore, under the restricted value condition, a principal may not choose to delegate authority in the first place, and may do away with the informed agent altogether if possible. Hence, what appears as a single-agent problem may only appear so because of incentive problems the principal seeks to avoid.

%In Section~\ref{sec:res_distortion}, we consider the restricted distortion condition, and show that no simple optimal strategy generally exists. In particular, we show that the delegation problem under restricted distortion is APX-hard. Unlike in the general case, however, we show that there are simple strategies that are \emph{approximately optimal} for the principal. Since the distortion of each action is state-independent, the principal may sort actions by their distortion, and restrict the agent to actions with low distortion, i.e. below some threshold. In the procurement example, this takes the form of a budget imposed on the agent. We show that the best such threshold policy is a $O(\log \pmin^{-1})$-approximation, where $\pmin$ is the probability of the least likely state. Hence, the performance of simple policies degrades smoothly with the degree of uncertainty faced by the principal. We also show in Section~\ref{sec:special} that when distortions are nonpositive and agent utilities are nonnegative, this improves to a $2$-approximation.

\paragraph{On Decomposition Coefficients} For the remainder of the paper, we assume $a_1=a_2=a_3=a_4=1$, and assume restricted value or distortion hold with respect to these coefficients. We do so only for simplicity of exposition. All results extend straightforwardly to any other nontrivial choice of decomposition coefficients. In particular, our approximation results hold with the same factors for any choice of decomposition coefficients.



==> general.tex <==
As a first result, we analyze the delegation problem in full generality, and conclude that it is not tractable. We show that the problem is hard to approximate within any sublinear factor. This holds even if the \blue{distribution over the states is uniform,} the principal's utility is binary (zero or one), and the agent's utility is limited to three different values. It is hence unreasonable to expect simple mechanisms which perform well in general.
\begin{theorem}\label{thm:general}
The delegation problem is NP-hard and also hard to approximate within any factor less than $\min\{m,n\}$.
\end{theorem}
\begin{proof}
We reduce from the Maximum Independent Set (MIS) problem. Given an instance of the MIS problem $\Gt=(\Vt,\Et)$\footnote{Throughout the paper, we use calligraphic letters for graph instances to distinguish between $\Vt$ (set of vertices) and $V$ (value matrix in delegation instance).} with $\abs{\Vt}=N$, we build an instance of the delegation problem with $N$ actions and $N$ states; i.e., one action and one state corresponding to each vertex of $\Gt$. \blue{We also assume that the states happen with the same probability $1/N$.} We set the utility of the principal to be the identity matrix, i.e., $\Up=\mathbb{I}_{N\times N}$. For the agent, the utility of action $i$ at state $j$ is defined by:
\begin{equation}
\Ua(i,j)=
\begin{cases}
1 & \quad \text{if $i=j$}, \\
2 & \quad \text{if $\{i,j\}\in \Et$}, \\
0 & \quad \text{otherwise.}
\end{cases}
\end{equation}
Choosing a set of actions by the principal can be thought as choosing a subset $\St\subseteq \Vt$. We claim that the utility of the principal is less than or equal to \blue{$\abs{\St}/N$}, with equality if and only if $\St$ is an independent set in $\Gt$. The inequality is clear because at each state $i \in \St$, the principal can get at most one by the choice of $\Up$ (and zero in other states). For the equality to occur, the agent should choose the action $i$ at each state $i\in \St$. This requires that no neighbor of $i$ is available, and hence $\St$ is an independent set.

By the previous argument, the maximum independent set maximizes the utility of the principal. On the other hand, given a solution of the delegation problem with (principal's) utility value $k/N$, one can find an independent set of size $k$ (by just selecting the states where the utility of the principal is non-zero). This implies that our reduction also preserves the objective values \blue{(besides normalizing by $N$).} Therefore, delegation inherits the hardness of approximation of the MIS problem \cite{haastad1999clique,zuckerman2006linear}.
\end{proof}


==> healthcare.tex <==
We now consider the case of restricted \d\ where the \d\ matrix is nonpositive. For ease of technical exposition, we consider the equivalent formulation 
\begin{equation}
\Up=V-D,\quad \Ua=V+D,
\end{equation}
where $V$ and $D$ are both non-negative matrices, and we have the following assumption on \d\ matrix.

\begin{assumption}[Restricted Distortion, Positive Bias]
The \d\ matrix $D$ is independent of the states and only a function of the actions. In other words,
$$d_{ij}=d_i\geq 0 \quad \forall j\in S.$$
\end{assumption}

With positive bias, the restricted distortion assumption is most often relevant when there are costs incurred by the principal which are less sensitive to the state than the mutual benefit derived from both players by actions. Example scenarios include managerial decisionmaking, where the firm pays the costs of the project selected by an informed agent in the firm, or when a manager seeks to hire new candidates, and observes information on the candidates via interviews.

As before, we prove upper- and lower-bounds on the approximability of the delegation problem under our assumption. For a lower bound, we prove APX-hardness in a similar manner to the result of Theorem~\ref{thm:APX_auction}. As an upper bound, we prove that there exists a threshold policy for the principal which guarantees a $O(\log n)$-approximation to the optimal utility. We also show that our analysis is tight, with a family of examples where no threshold policy can achieve better than a logarithmic approximation factor. For the positive bias setting, thresholds take the form of caps on the allowable distortion of actions offered to the agent. For applications such as those described above, this suggests the practicality of spending caps or budgets for the agent as a form of managerial control. We formalize our results below, beginning with our hardness result.

\begin{theorem}
Under \healthcare\ with restricted \d\ matrix, the delegation problem is APX-hard.
\end{theorem}

\begin{proof}
The proof is similar to Theorem~\ref{thm:APX_auction}. See Appendix~\ref{supp:APX_healthcare} for details.
\end{proof}
 We now turn to our approximation result. Before delving into the algorithm, we give some insight on the difference between \auction\ and \healthcare, which impedes a similar constant-factor approximation. In particular, one can mimic equation~\eqref{eq:auction_intuition} by writing:
$$\Up=V-D=(V+D)-2D=\Ua-2D,$$
where again we can optimize them individually. More precisely, we can maximize the utility of the agent by allowing the entire set of actions; and we can minimize the \d\ (i.e., maximize $-2D$ part) by allowing the single action with lowest \d. Since we are maximizing the difference in this case (equivalently, since we do not have non-negativity assumption for the second contributive part), the individual maximizers do not necessarily provide a good approximation for the entire utility.
%
%\begin{example}
%Consider an example with $m=3$ actions and only $n=1$ state, with the following matrices:
%\begin{equation}
%V=\left[ \begin{array}{c}
%   \epsilon\\
%   3\\
%   2+\epsilon
%\end{array}\right ],\quad 
%D=\left[ \begin{array}{c}
%   0\\
%   1\\
%   2
%\end{array}\right ].
%\end{equation}
%The optimal solution is to allow second action which gives a utility of $2$ to the principal. On the other hand, allowing all actions or lowest-\d\ action will result in only $\epsilon$ utility.
%\end{example}
%
%To resolve this issue, note that in the previous example, the reason why the entire set $\Omega$ failed to give a good utility was the existence of a high-\d\ action (third action) with a \v\ slightly bigger than its \d. Instead of discarding this candidate solution, we can start modifying it by removing high-\d\ actions one by one, in the order of decreasing \d. For example, once we remove the third action from $\Omega=\{1,2,3\}$ in the above example, we get an optimal delegation set. It is also possible (for general $n$) that we lose utility in other states as we remove high-\d\ actions, but through a balance between the \d\ cap and utility loss we can hope to get a good result. It turns out that this simple strategy gives an approximate solution in general, which is analyzed in the following theorem.

Nonetheless, we show that if the principal considers every threshold strategy and chooses the best, they are guaranteed at least a $2\log(n)$-approximation to their utility under the optimal mechanism. We formalize this policy in Algorithm~\ref{alg:healthcare}, and analyze its performance in Lemma~\ref{lemma:part_one} and Theorem~\ref{thm:healthcare}. We further show that this analysis is essentially tight, by giving a family of examples where no threshold achieves better than a $\Omega(\log n)$-approximation. Formally, we prove:

\begin{theorem}\label{thm:healthcare}
	Algorithm~\ref{alg:healthcare} is a $2\log{n}$-approximation algorithm\footnote{Logarithms are with respect to base $2$.} under the \healthcare\ assumption with restricted \d\ matrix.
\end{theorem}

\begin{theorem}\label{thm:hclower}
	There exists a family of instances where no threshold policy is better than a $\Omega(\log n)$-approximation.
\end{theorem}

%============= Algorithm ============
\begin{algorithm}[t]
	\SetAlgoNoLine
	\KwIn{Set of actions $\Omega$, set of states $S$, \v\ ($V$) and \d\ ($D$) matrices.}
	\KwOut{Set of actions $A$ that approximately maximizes $f(A)$.}
	$\Up=V-D$, $\Ua=V+D$.\\
	\For{each $k\in \{1,2,...,m\}$}{
	$threshold=d_k$.\\
	Set $A_k\gets \{i\in \Omega:d_i\leq threshold\}$.
		}
	Let $\mathcal{A}\coloneq\{A_1,...,A_m\}$.\\
	{\bf Return} $\argmax_{A\in \mathcal{A}} f(A)$.\\
	\caption{Restricted Distortion, Positive Bias Delegation}
	\label{alg:healthcare}
\end{algorithm}
%=================================

We prove Theorem~\ref{thm:healthcare} in the sequel, and argue Theorem~\ref{thm:hclower} in Appendix~\ref{supp:APX_healthcare}. Our upper bound for positive bias delegation relies on partitioning the set of states into two subsets of high and low distortion. Let $OPT$ be the optimal solution and $d_\text{max}=\max_{i\in OPT} d_i$ be the highest \d\ in $OPT$.\footnote{Interchangeably, we use $OPT$ ($APX$) to denote both the optimal (approximate) set of actions that the principal should allow, and also the optimal (approximate) utility that he achieves by doing so.} We will ignore actions with higher distortion than $d_\text{max}$, as we may achieve the desired approximation guarantee while doing so.

Let $\Delta>0$ be a constant to be selected shortly. We say that a state is \emph{high-\d} (HD) if $OPT$ chooses an action with \d\ $d\in [d_\text{max}-\Delta,d_\text{max}]$ in that state, and otherwise the state is called \emph{low-\d} (LD). These definitions give a partition of the states into two sets $\Sexp$ and $\Scheap$ with sizes $n_1$ and $n_2$ such that $S=\Sexp\cup \Scheap$, and $n_1+n_2=n=\abs{S}$. As $n_1$ and $n_2$ are increasing and decreasing functions of $\Delta$, respectively, there exists a $\Delta$ such that $n_1=n_2=n/2$.\footnote{In the case of odd $n$, the arguments hold by choosing $\Delta$ such that $n_1=\lfloor{n/2}\rfloor$ and $n_2=\lceil{n/2}\rceil$. For simplicity of exposition, we assume that $n$ is even. If there is no value of $\Delta$ where in $n_1+n_2=n$, then there is a jump in $n_1$ at some $\Delta=\Delta_0$. Then there are $k$ states in which the action picked by the agent has \d\ equal to $d_\text{max}-\Delta_0$. In that case, we can pick $\Delta_0$ as our \d\ margin ($\Delta$) and divide those $k$ states between $\Sexp$ and $\Scheap$ such that they have the desired sizes.} Choose $\Delta$ such that this holds.

Let $\OPTexp$ and $\OPTcheap$ be the utility of the principal from each partition, i.e.,
\begin{equation}
\OPTexp=\sum_{i\in \Sexp} (v_{a_i,i}-d_{a_i}),\quad \quad \OPTcheap=\sum_{i\in \Scheap} (v_{a_i,i}-d_{a_i}),
\end{equation}
where $a_i$ is the index of the action that $OPT$ picks in state $i$, and clearly $OPT=\OPTexp+\OPTcheap$.
The following lemma states that the portion of principal's optimal utility ($OPT$) coming from high-distortion states can be approximated up to a constant factor, by picking the better of two threshold solutions.

%%%%%%%%%%%%%%%%%% Lemma %%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lemma:part_one}
Let $APX_1=\{i\in \Omega:d_i\leq d_\text{max}\}$ and $APX_2=\{i\in \Omega:d_i\leq d_\text{max}-\Delta\}$, i.e., sets of actions that has \d\ no more than $d_\text{max}$ and $d_\text{max}-\Delta$, respectively.\footnote{Note that $d_\text{max}$ and $\Delta$ require knowledge of the optimal solution. They are being used solely for analysis, rather than as part of our algorithm.} Then:
$$\max{\{APX_1,APX_2\}}\geq \frac{1}{2}\OPTexp.$$
\end{lemma}

\begin{proof}
Let $b_i$ denote the action picked by the approximate solution (which can be either $APX_1$ or $APX_2$) in state $i$.
Considering $APX_1$, in each state $i\in S$ we have
$$v_{b_i,i}+d_{b_i}\geq v_{a_i,i}+d_{a_i},$$
since the agent decided to choose $b_i$, while $a_i$ was also allowed in $APX_1$. This implies the following helpful inequality which relates the loss in principal's utility to the \d\ difference of chosen actions:
\begin{equation}
v_{b_i,i}-d_{b_i}\geq v_{a_i,i}-d_{a_i}+2(d_{a_i}-d_{b_i}).
\label{eq:agent_choice}
\end{equation}
Equation~\eqref{eq:agent_choice} has the following interpretations: First, the principal gains (in a particular state $i$) if the agent picks an action with lower distortion in the approximate solution ($d_{b_i}\leq d_{a_i}$). Second, in case the agent picks an action with higher distortion than that of the optimal solution, the loss in principal's utility is bounded by twice the distortion difference. However, this difference is bounded by $\Delta$ in the high-\d\ states, because for $i\in \Sexp$ we have $d_{a_i}\geq d_\text{max}-\Delta\geq d_{b_i}-\Delta$, which implies
\begin{equation}
d_{b_i}-d_{a_i}\leq \Delta.
\label{eq:price_diff}
\end{equation}
Using these two inequalities we can get the following lower bound on $APX_1$:
\begin{subequations}
\begin{align}
APX_1 &=\sum_{i\in S}(v_{b_i,i}-d_{b_i})\geq \sum_{i\in \Sexp}(v_{b_i,i}-d_{b_i})\\
& \geq \sum_{i\in \Sexp}(v_{a_i,i}-d_{a_i}+2(d_{a_i}-d_{b_i}))\label{eq:APX1s2}\\ 
& \geq \sum_{i\in \Sexp}(v_{a_i,i}-d_{a_i}-2\Delta)=\OPTexp-2n_1\Delta=\OPTexp-n\Delta, \label{eq:APX1s3}
\end{align}
\end{subequations}
where in the first inequality we just restricted the summation to the set of high-\d\ actions, in \eqref{eq:APX1s2} we used inequality \eqref{eq:agent_choice}, and in \eqref{eq:APX1s3} we used inequality \eqref{eq:price_diff} and the fact that $n_1=n/2$.

Considering $APX_2$, we still have inequality \eqref{eq:agent_choice} for low-\d\ states, because by the definition of low-\d\ state, action $a_i$ has a \d\ no more than $d_\text{max}-\Delta$ and therefore it is allowed in $APX_2$. However, we need a new bound on the \d\ differences. Note that by the positivity assumption of utilities, the utility of the agent from picking the highest-\d\ action in $OPT$ is at least $2d_\text{max}$ (for all $i\in S$), hence any action that is picked in any state $i$ has to satisfy at least
$$v_{a_i,i}+d_{a_i}\geq 2d_\text{max},$$
which can be rearranged as
$$d_\text{max}-d_{a_i}\leq \frac{v_{a_i,i}-d_{a_i}}{2}.$$
Since we allow actions up to the \d\ of $d_\text{max}-\Delta$, we get this bound on the \d\ difference:
\begin{equation}
d_{b_i}-d_{a_i}\leq d_\text{max}-\Delta-d_{a_i}\leq \frac{v_{a_i,i}-d_{a_i}}{2}-\Delta.
\label{eq:price_diff_2}
\end{equation}
Now we can find a lower bound on $APX_2$.
\begin{subequations}
\begin{align}
APX_2 &=\sum_{i\in S}(v_{b_i,i}-d_{b_i})\geq \sum_{i\in \Scheap}(v_{b_i,i}-d_{b_i})\\
& \geq \sum_{i\in \Scheap}(v_{a_i,i}-d_{a_i}+2(d_{a_i}-d_{b_i}))\label{eq:APX2s2}\\ 
& \geq \sum_{i\in \Scheap}\left(v_{a_i,i}-d_{a_i}-2\big(\frac{v_{a_i,i}-d_{a_i}}{2}-\Delta\big)\right)=2n_2\Delta=n\Delta, \label{eq:APX2s3}
\end{align}
\end{subequations}
where this time we restricted the summation to the set of low-\d\ actions, in \eqref{eq:APX2s2} we used inequality \eqref{eq:agent_choice}, and in \eqref{eq:APX2s3} we used inequality \eqref{eq:price_diff_2} and the fact that $n_2=n/2$.

We finish the proof by showing that the better solution among $APX_1$ and $APX_2$ is a 2-approximation for $\OPTexp$.
$$\max{\{APX_1,APX_2\}}\geq \frac{1}{2}(APX_1+APX_2)\geq \frac{1}{2}(\OPTexp-n\Delta+n\Delta)=\frac{1}{2}\OPTexp.$$
\end{proof}
Now we are ready to analyze the performance of Algorithm~\ref{alg:healthcare}. We use an inductive argument to show that the previous 2-approximation of $\OPTexp$ implies an $O(\log{n})$-approximation for $OPT$.

%%%%%%%%%%%%%%%%%% Theorem %%%%%%%%%%%%%%%%%%%%%%%%


\begin{proof}[Proof of Theorem~\ref{thm:healthcare}]
We prove by induction (on the number of states) that there exists a $2\log{n}$-approximation algorithm for $OPT$. Intuitively, if $\OPTexp$ is the dominant part of $OPT$, then $\max{\{APX_1,APX_2\}}$ from Lemma~\ref{lemma:part_one} is a good approximation for $OPT$ too. On the other hand if $\OPTcheap$ is dominant, we can ignore all the high-\d\ states without losing much, and this reduces the number of states by half. 

%For the base case where we only have $n=1$ state, we can exactly solve the problem by checking all singletons (i.e., allowing only one action in each solution). 
For the base case, we show that there exists a $2$-approximation for $n=2$ states. Clearly, one of the states generates at least half of the utility in the optimal solution (i.e., $OPT/2$). Let $i^*\in \{1,2\}$ be that particular state, and $a_{i^*}$ be the corresponding action in the optimal solution. The solution that consists of $a_{i^*}$ and all actions with lower \d\ will be a $2$-approximation. It is guaranteed to generate at least $OPT/2$ utility in state $i^*$, because it cannot go to higher \d\ levels and its utility will be at least equal to what $OPT$ provides, based on \eqref{eq:agent_choice}.


Now assume that we have a $2\log{\frac{n}{2}}$-approximation for any problem with $n/2$ states. For the problem with $n$ states, one of the following happens:\\

\noindent {\bf Case I (Dominant $\OPTexp$).} If we have $\OPTexp\geq \frac{1}{\log{n}}OPT$, then
$$\max{\{APX_1,APX_2\}}\geq \frac{1}{2}\OPTexp\geq \frac{1}{2\log{n}}OPT,$$
which is the desired approximation ratio.
\\\\
\noindent {\bf Case II (Dominant $\OPTcheap$).} In this case we have the opposite assumption $\OPTexp< \frac{1}{\log{n}}OPT$, which implies:
$$\OPTcheap\geq \left(1-\frac{1}{\log{n}}\right)OPT=\frac{\log{n/2}}{\log{n}}OPT.$$
Now using the $2\log{\frac{n}{2}}$-approximation (inductive assumption) on the set $\Scheap$ will give a solution $APX^\text{LD}$ such that
$$APX^\text{LD}\geq \frac{1}{2\log{n/2}}\OPTcheap.$$
Combining the two inequalities we get:
$$APX^\text{LD}\geq \frac{1}{2\log{n/2}}\times \frac{\log{n/2}}{\log{n}}OPT=\frac{1}{2\log{n}}OPT,$$
which again gives the desired approximation ratio.

Finally, note that even though $d_\text{max}$, $\Delta$, $\Scheap$, and $\Sexp$ in the \ proof are all defined based on the optimal solution and hence are not known, all the proposed approximate solutions (i.e., $APX_1$, $APX_2$, or the base case solution) have a simple structure. There exists a \d\ threshold such that every action with lower \d\ is allowed, and everything else is excluded. Therefore, the approximate delegation solution can be found by the linear-time search of Algorithm~\ref{alg:healthcare}. This proves the theorem.
\end{proof}

\paragraph{Matching lower bound.}  
We conclude by emphasizing that the above analysis is tight. We show in Appendix~\ref{supp:log_lower_bound} that our analysis in Theorem~\ref{thm:healthcare} is tight up to a constant factor. We do so by providing instances where no threshold policy can outperform the logarithmic approximation ratio.


==> nonuniform.tex <==
We now extend the approximation result for restricted distortion from uniformly distributed to arbitrarily distributed states. We do so via a reduction that loses a factor of $2$. For uniformly distributed states, the approximation ratio depended on the number of states. For non-uniform states, the natural analog is the inverse of the probability of the least likely state.

 Let $U_P$, $U_A$ be an instance of the delegation with states distributed according to $(p_1,\ldots, p_n)$. Let $\pmin=\min_{s\in S}p_s$ be the probability of the least likely state. We will construct a new instance of the problem with the same actions, a new set of uniformly distributed states, and where the principal's utility from any delegation set is within a constant factor in the two instances. The number of states in the new instance will be at most $\pmin^{-1}$. Furthermore, if the original instance satisfied restricted distortion, so too will the new instance.

The rough approach to the reduction will be rounding each state's probability down to the nearest factor of $\pmin$ (and normalizing). Doing so will distort the utility from any delegation set by at most a factor of $2$. We may then divide each state evenly into many identical copies which each occur with probability $\pmin$.

Formally, for each state $s$, let $\bar p_s=\pmin\lfloor p_s/\pmin\rfloor$ be $p_s$ rounded down to the nearest factor of $\pmin$. In our new instance, we will replace $s$ with $k(s)=\lfloor p_s/\pmin\rfloor$ identical states, labeled $s^1,\ldots, s^{k(s)}$. The new probabilities will be given by $p'_{s^1}=p'_{s^2}=\ldots = p'_{s^{k(s)}}=\pmin/c$, where $c=\sum_{s\in S}\bar p_s$ is a normalizing constant to ensure probabilities sum to $1$. Our new utilities will be given by $\Up '(a,s^i)=c\Up(a,s)$ and $\Ua '(a,s^i)=c\Ua(a,s)$ for all $a\in \Omega$, $s\in S$, and $i\in \{1,\ldots, k(s)\}$. Note that in state $s^i$ for any $s$ and $i\in\{1,\ldots, k(s)\}$, the agent's preferences over actions are identical to their preferences in state $s$ of the original instance. We now show that because $\pmin$ was smaller than all other probabilities, rounding in the manner discussed does not distort utilties significantly for the principal. In particular:

\begin{lemma}\label{lem:unifreduct}
For any delegation set $A$, let $f(A)$ denote the principal's utility from $A$ in the original instance, and $f'(A)$ the principal's utility from $A$ in the transformed instance. The following inequality holds:
\begin{equation*}
2 f'(A) \geq f(A) \geq f'(A).
\end{equation*}
\end{lemma}
\begin{proof}
We first prove $f(A)\geq f'(A)$. We have:
\begin{align*}
	f'(A)&=\sum_{s\in S} \sum_{i=1}^{k(s)}p'_{s^i}\Up'(g(A,s^i),s^i)\\
	&=\sum_{s\in S}\bar p_s \Up(g(A,s),s)\\
	&\leq \sum_{s\in S}p_s \Up(g(A,s),s)=f(A)
\end{align*}
In fact, if we show $2\bar p_s\geq p_s$ for all $s\in S$, then the above analysis also implies $2f'(A)\geq f(A)$. This latter fact follows from the observation that $p_s-\bar p_s\leq \pmin\leq \bar p_s$.
\end{proof}

The above mapping from delegation instances with arbitrarily distributed states to those with uniformly distributed states immediately implies that we may use approximation algorithms from the latter setting to obtain approximately optimal solutions to the former. This will immediately yield Theorem~\ref{thm:uniform} as a corollary. Formally:

\begin{theorem}
	Let $\alpha(\cdot)$ be a nondecreasing function that is at least $1$. Then for any $\alpha(n)$-approximation algorithm for delegation instances with uniformly distributed states, there exists a  $2\alpha(\pmin^{-1})$-approximation algorithm for delegation instances with arbitrarily distributed states.
\end{theorem}
\begin{proof}
Let an approximation algorithm for uniform states be given. Consider running the algorithm in question on the uniform instance constructed above, and let $A$ and $A^*$ be the set of actions produced by the algorithm and an optimal solution, respectively. Further let $A'$ denote an optimal solution to the uniform instance. Note that the number $n'$ of states in the uniform instance is at most $\pmin^{-1}$. By Lemma~\ref{lem:unifreduct}, the we have the following sequence of inequalities, which implies the result.
\begin{equation*}
f(A)\geq f'(A)\geq \tfrac{1}{\alpha(n')}f'(A')\geq \tfrac{1}{\alpha(\pmin^{-1})}f'(A')\geq \tfrac{1}{\alpha(\pmin^{-1})}f'(A^*)\geq \tfrac{1}{2\alpha(\pmin^{-1})}f(A^*).
\end{equation*}
\end{proof}

We conclude by re-emphasizing that Theorem~\ref{thm:uniform} is asymptotically tight. The uniform states example in Appendix~\ref{supp:lognlb} also applies in the more general setting of non-uniform states. Moreover, note that combining identical states yields an example with many fewer states, ruling out the possibility of an approximation factor which depends only on the number of states and not their distribution.


\subsection{Computational Hardness}
In this Section, we briefly note that with restricted distortion and no independence, the principal's delegation is computationally intractable in a fairly strong sense: there exists some constant threshold such that delegation is NP-hard to approximate better than that constant, i.e. it is APX-Hard.

\begin{theorem}
	\label{thm:APX_hardness}
	If utilities satisfy restricted distortion condition, the principal's delegation problem is APX-hard, even under uniformly distributed states.
\end{theorem}

\begin{proof}

We give a reduction from the bounded degree vertex cover problem, i.e., the vertex cover problem on graphs with degree at most $B$ (constant). This problem is known to be APX-hard \cite{clementi1999improved}. Consider an instance of the bounded degree vertex cover problem $\Gt=(\Vt,\Et)$ with $\nt$ nodes and $\mt$ edges (where $\mt\leq B\cdot\nt/2=\O(\nt)$).\footnote{To distinguish between the parameters of the vertex cover instance and the delegation instance, we use tilde ($\sim$) for the graph instance.} We construct an instance of the delegation problem with $\mt+\nt$ states and $\nt+1$ actions, in which the distribution over states is uniform. For each node $i$, there is an action $a_i$, with an additional ``default'' action $a_0$. Regarding states, there is a state $s_e$ for each edge $e=\{i,j\}$, whose value is $5$ only for actions $a_i$ and $a_j$ (two ends of that edge), $2$ for the default action, and $0$ for all other actions. There is also a state $s_i$ for each node $i$, whose value is $2$ only for $a_i$ and $a_0$ (default action), and $0$ for all other actions. Moreover, the only action with non-zero \d\ is the default action with $d_0=-1$.

We claim that the optimal solution of the delegation problem produces a utility of $(5\mt+3\nt-\kt)/(\mt+\nt)$ for the principal, where $\kt$ is the size of the smallest vertex cover of $\Gt$. To see this, first note that any solution $\St \subseteq \Vt$ can be improved by including $a_0$, since $a_0$ has {a negative distortion}. Any time the agent would choose $a_0$, it is the optimal choice for the principal as well. We therefore only consider solutions containing $a_0$.

Now if $\St$ is a vertex cover of $\Gt$ with $\abs{\St}=\kt$, consider the corresponding delegation set where the principal allows actions $\{a_i: i\in \St\}\cup\{a_0\}$. In all the states corresponding to edges, the agent will pick the action corresponding to one end of that edge (one is guaranteed to be in the cover $\St$) to get a utility of $5$ compared to $2-1$ achievable from the default action. This choice will also generate utility of $5$ for the principal, which makes $5\mt$ in total. For the states $s_i, i\in \St$ the agent will pick action $a_i$ which generates the utility of $2$ for both principal and agent. This will make $2\kt$ in total. Finally, for states $s_i,i\in \Vt\backslash\St$ the agent picks the default action which generates a utility of $2-1$ for himself but $2+1$ for the principal. This will give $3(\nt-\kt)$ in total. Summing up the utilities and dividing by the number of states will give $(5\mt+3\nt-\kt)/(\mt+\nt)$.

For the converse, consider an optimal solution $A$ to the delegation problem. We show that the nodes corresponding to the actions in $A$ (excluding the default action) induce a vertex cover; otherwise the solution can be improved. Assume that there exists an edge $e=\{i,j\}$ where neither $a_i$ nor $a_j$ is allowed in $A$. If we add action $a_i$ to $A$, the principal gets a utility of $5$ in state $s_e$, compared to current utility of $3$ from the default action. On the other hand, the utility of the principal decreases in state $s_i$ from $3$ to $2$. So the total utility of $A\cup\{a_i\}$ is more than $A$ which contradicts the optimality of $A$. Therefore $A$ should be a vertex cover (plus default action). This in turn implies that the utility is at most $(5\mt+3\nt-\kt)/(\mt+\nt)$ where $\kt$ is the size of the minimum vertex cover.

Since $\mt=\Theta(\nt)$ and the minimum vertex cover has size at least $\mt/B=\Omega(\nt)$, a constant factor gap in the bounded degree vertex cover problem translates into a constant factor gap in the optimal solution of the delegation problem, which yields the desired APX-hardness result. 
\end{proof}
%While Theorem~\ref{thm:APX_hardness} rules out mechanisms which are both simple and optimal, it does not rule out mechanisms which are simple and \emph{approximately optimal}. Our second result of this section is that such mechanisms generally exist. Under the restricted distortion condition, it is possible to rank actions based on their distortion. The most natural, simple class of delegation mechanisms to analyze, then, is \emph{threshold policies}, which include actions with distortion below a certain level, and exclude those above. Since there are polynomially many such thresholds, analyzing the performance of best threshold is of special interest. We formalize this in Algorithm~\ref{alg:healthcare}.

==> results.tex <==
Our contributions are as follows.
\begin{itemize}
	\item We introduce a discrete model for delegation. We prove that optimal delegation in the fully general formulation of this model is NP-hard to approximate within any factor which is sublinear in the number of states or actions.
	\item Given a delegation instance we show how to quantify the misalignment in incentives for each pair of state and actions, detailed in Section~\ref{sec:decomp}. We study the case where this misalignment measure is restricted in its state-dependence.
	\item In Section~\ref{sec:indep}, we analyze the case where misalignment is insensitive to state and utilities are independent across actions. We show that threshold policies secure for the principal a constant-approximation of the utility from the optimal mechanism.
	\item In Section~\ref{sec:res_distortion} we maintain the assumption of state-insensitive misalignment, but relax the assumption of independence. We give matching (up to a constant) upper and lower bounds on the performance of threshold policies that degrade logarithmically with the complexity of the state space.
	\item In Section~\ref{sec:res_agreement}, we give a supplementary analysis of a related setting where action-specific {\em alignment} of preferences is insensitive to state, while biases may depend on state. We show that depending on the presence or absence of an outside option for the agent, the delegation problem is either computationally intractable or solvable exactly by the principal imposing the best action on the agent, respectively.
	\item We give several additional results for, the setting of Section~\ref{sec:res_distortion}, including computational hardness results and an additional constant-approximation with out independence assuming nonnegative agent utility.
\end{itemize}
A notable application of our results is assortment selection with a unit-demand agent. In the literature on assortment selection, it is common to study utility-based models of buyer choice, e.g. multinomial logit \cite{MMVZ14}. The results of Section~\ref{sec:res_distortion} apply to all such settings, and with independence (as in multinomial logit), the results in Section~\ref{sec:indep} imply a constant-approximation. Both sets of results are new to this literature.

==> special.tex <==
We finally note two additional assumptions which together immediately imply threshold policies are a \emph{constant}-approximation in the restricted distortion case. First, throughout the paper we have assumed that the principal's utility for every action and every state was nonnegative; this was to make approximation sensible. For the agent, on the other hand, the sign of their utility was not important. The only thing that mattered was their preference ordering over actions in each state. In this section, we add the assumption that the agent's utilities are also nonnegative, i.e. $\Ua(a,s)\geq 0$ for all $a\in \Omega$ and $s\in S$.

Second, we note that prior to this section, the utility decomposition might yield distortions which are negative. In some settings, distortions are nonpositive. This might occur, for example, if distortions take the form of transfers from the agent to the principal, or as costs felt only by the agent. In this section, we assume that $d_a\leq 0$ for all $a\in \Omega$.

Under these two assumptions (and taking the decomposition with coefficients $a_1=a_2=a_3=a_4=1$), we may write $U_P=V+D-2D$. The agent's utility is given by $V+D$, and is maximized by the threshold strategy that offers the full set of actions. Meanwhile, selecting the action with the most negative distortion maximizes the term $-2D$, and is also a threshold strategy. This yields a simple argument that threshold strategies are a $2$-approximation. In fact, a more nuanced characterization can be obtained, and is summarized in the following two theorems, proved in Appendices~\ref{supp:improved} and~\ref{supp:lower_bound}.

\begin{theorem}
\label{thm:improved}
There always exists a threshold which is a $(2-\pmin)$-approximation for the delegation problem under restricted distortion assumption, when the distortions are nonpositive and the agent's utilities are nonnegative.
\end{theorem}

\begin{theorem}
	\label{thm:lower_bound}
	There exists a family of instances satisfying restricted, nonpositive distortion and nonnegative agent utilities such that the best threshold is at best a $(2-\pmin)$-approximation.
\end{theorem}

==> wologapp.tex <==
We consider first the restricted value case. We first consider the case where $a_2>0$, and then relax this assumption. Given $(a_1,a_2,a_3,a_4,V,D)$, let $V'=\tfrac{a_1a_4-a_2a_3}{2a_2}V$ and $D'=\tfrac{a_1a_4+a_2a_3}{2a_2}V+a_4D$. We then have:
\begin{equation*}
U_P'=\frac{a_1a_4}{a_2}V-a_4D=V'-D'
\end{equation*}

